Sobolev and BV spaces on metric measure spaces via derivations and integration by parts

We develop a theory of BV and Sobolev Spaces via integration by parts formula in abstract metric spaces; the role of vector fields is played by Weaver's metric derivations. The definition hereby given is shown to be equivalent to many others present in literature.

==> macro2010.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                         %%
%%     SIMBOLI GENERALI (che di solito uso per tutti i lavori)             %%
%%                                                                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%
%%     SIMBOLI MATEMATICI BLACKBOARD (INSIEMI) R -> \R
%%
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
%%
%%
%%     SIMBOLI MATEMATICI CALLIGRAFICI SCRIPT      R -> \RR
%%
%%
\renewcommand{\AA}{\mathscr{A}}
\newcommand{\BB}{\mathscr{B}}
\newcommand{\DD}{\mathscr{D}}
\newcommand{\EE}{\mathscr{E}}
\newcommand{\FF}{\mathscr{F}}
\newcommand{\GG}{\mathscr{G}}
\newcommand{\HH}{\mathscr{H}}
\newcommand{\LL}{\mathscr{L}}
\newcommand{\MM}{\mathscr{M}}
\newcommand{\PP}{\mathscr{P}}
\renewcommand{\SS}{\mathscr{S}}
\newcommand{\TT}{\mathscr{T}}
\newcommand{\VV}{\mathscr{V}}
\newcommand{\WW}{\mathscr{W}}
%%
%%
%%
%%         SIMBOLI MATEMATICI CALLIGRAFICI  CAL  R -> \cR
%%
%%
\newcommand{\cA}{{\ensuremath{\mathcal A}}}
\newcommand{\cB}{{\ensuremath{\mathcal B}}}
\newcommand{\calC}{{\ensuremath{\mathcal C}}}
\newcommand{\cD}{{\ensuremath{\mathcal D}}}
\newcommand{\cE}{{\ensuremath{\mathcal E}}}
\newcommand{\cF}{{\ensuremath{\mathcal F}}}
\newcommand{\cG}{{\ensuremath{\mathcal G}}}
\newcommand{\cH}{{\ensuremath{\mathcal H}}}
\newcommand{\cK}{{\ensuremath{\mathcal K}}}
\newcommand{\cL}{{\ensuremath{\mathcal L}}}
\newcommand{\cM}{{\ensuremath{\mathcal M}}}
\newcommand{\cN}{{\ensuremath{\mathcal N}}}
\newcommand{\cO}{{\ensuremath{\mathcal O}}}
\newcommand{\cP}{{\ensuremath{\mathcal P}}}
\newcommand{\cT}{{\ensuremath{\mathcal T}}}
\newcommand{\cX}{{\ensuremath{\mathcal X}}}
\newcommand{\cY}{{\ensuremath{\mathcal Y}}}
\newcommand{\cV}{{\ensuremath{\mathcal V}}}
\newcommand{\cW}{{\ensuremath{\mathcal W}}}
%%
%%
%%
%%     SIMBOLI MATEMATICI BOLD (raddoppiano l'iniziale)  a -> \aa,  B -> \bB,
%%     \gamma -> \ggamma
%%     quando sono apici o pedici si aggiunge una s
%%     a -> \saa, \beta -> \sbbeta
%% 
%% 
\renewcommand{\aa}{{\mbox{\boldmath$a$}}}
\newcommand{\bb}{{\mbox{\boldmath$b$}}}
\newcommand{\cc}{{\mbox{\boldmath$c$}}}
\newcommand{\dd}{{\mbox{\boldmath$d$}}}
\newcommand{\ee}{{\mbox{\boldmath$e$}}}
\newcommand{\ff}{{\mbox{\boldmath$f$}}}
\renewcommand{\gg}{{\mbox{\boldmath$g$}}}
\newcommand{\hh}{{\mbox{\boldmath$h$}}}
\newcommand{\ii}{{\mbox{\boldmath$i$}}}
\newcommand{\jj}{{\mbox{\boldmath$j$}}}
\newcommand{\mm}{{\mbox{\boldmath$m$}}}
\newcommand{\nn}{{\mbox{\boldmath$n$}}}
\newcommand{\oo}{{\mbox{\boldmath$o$}}}
\newcommand{\pp}{{\mbox{\boldmath$p$}}}
\newcommand{\qq}{{\mbox{\boldmath$q$}}}
\newcommand{\rr}{{\mbox{\boldmath$r$}}}
\renewcommand{\ss}{{\mbox{\boldmath$s$}}}
\renewcommand{\tt}{{\mbox{\boldmath$t$}}}
\newcommand{\uu}{{\mbox{\boldmath$u$}}}
\newcommand{\vv}{{\mbox{\boldmath$v$}}}
\newcommand{\ww}{{\mbox{\boldmath$w$}}}
\newcommand{\xx}{{\mbox{\boldmath$x$}}}
\newcommand{\yy}{{\mbox{\boldmath$y$}}}
\newcommand{\zz}{{\mbox{\boldmath$z$}}}
%%
%%
\newcommand{\saa}{{\mbox{\scriptsize\boldmath$a$}}}
\newcommand{\sbb}{{\mbox{\scriptsize\boldmath$b$}}}
\newcommand{\scc}{{\mbox{\scriptsize\boldmath$c$}}}
\newcommand{\sdd}{{\mbox{\scriptsize\boldmath$d$}}}
%\newcommand{\see}{{\mbox{\scriptsize\boldmath$e$}}}
\newcommand{\sff}{{\mbox{\scriptsize\boldmath$f$}}}
\newcommand{\sgg}{{\mbox{\scriptsize\boldmath$g$}}}
\newcommand{\shh}{{\mbox{\scriptsize\boldmath$h$}}}
\newcommand{\sii}{{\mbox{\scriptsize\boldmath$i$}}}
\newcommand{\sjj}{{\mbox{\scriptsize\boldmath$j$}}}
\newcommand{\smm}{{\mbox{\scriptsize\boldmath$m$}}}
\newcommand{\snn}{{\mbox{\scriptsize\boldmath$n$}}}
\newcommand{\soo}{{\mbox{\scriptsize\boldmath$o$}}}
\newcommand{\spp}{{\mbox{\scriptsize\boldmath$p$}}}
\newcommand{\sqq}{{\mbox{\scriptsize\boldmath$q$}}}
\newcommand{\srr}{{\mbox{\scriptsize\boldmath$r$}}}
\newcommand{\sss}{{\mbox{\scriptsize\boldmath$s$}}}
\newcommand{\stt}{{\mbox{\scriptsize\boldmath$t$}}}
\newcommand{\suu}{{\mbox{\scriptsize\boldmath$u$}}}
\newcommand{\svv}{{\mbox{\scriptsize\boldmath$v$}}}
\newcommand{\sww}{{\mbox{\scriptsize\boldmath$w$}}}
\newcommand{\sxx}{{\mbox{\scriptsize\boldmath$x$}}}
\newcommand{\syy}{{\mbox{\scriptsize\boldmath$y$}}}
\newcommand{\szz}{{\mbox{\scriptsize\boldmath$z$}}}
%%
%%
%%
\newcommand{\aA}{{\mbox{\boldmath$A$}}}
\newcommand{\bB}{{\mbox{\boldmath$B$}}}
\newcommand{\cC}{{\mbox{\boldmath$C$}}}
\newcommand{\dD}{{\mbox{\boldmath$D$}}}
\newcommand{\eE}{{\mbox{\boldmath$E$}}}
\newcommand{\fF}{{\mbox{\boldmath$F$}}}
\newcommand{\gG}{{\mbox{\boldmath$G$}}}
\newcommand{\hH}{{\mbox{\boldmath$H$}}}
\newcommand{\iI}{{\mbox{\boldmath$I$}}}
\newcommand{\jJ}{{\mbox{\boldmath$J$}}}
\newcommand{\mM}{{\mbox{\boldmath$M$}}}
\newcommand{\nN}{{\mbox{\boldmath$N$}}}
\newcommand{\oO}{{\mbox{\boldmath$O$}}}
\newcommand{\pP}{{\mbox{\boldmath$P$}}}
\newcommand{\qQ}{{\mbox{\boldmath$Q$}}}
\newcommand{\rR}{{\mbox{\boldmath$R$}}}
\newcommand{\sS}{{\mbox{\boldmath$S$}}}
\newcommand{\tT}{{\mbox{\boldmath$T$}}}
\newcommand{\uU}{{\mbox{\boldmath$U$}}}
\newcommand{\vV}{{\mbox{\boldmath$V$}}}
\newcommand{\wW}{{\mbox{\boldmath$W$}}}
\newcommand{\xX}{{\mbox{\boldmath$X$}}}
\newcommand{\yY}{{\mbox{\boldmath$Y$}}}
%%
%%
%%
\newcommand{\saA}{{\mbox{\scriptsize\boldmath$A$}}}
\newcommand{\sbB}{{\mbox{\scriptsize\boldmath$B$}}}
\newcommand{\scC}{{\mbox{\scriptsize\boldmath$C$}}}
\newcommand{\sdD}{{\mbox{\scriptsize\boldmath$D$}}}
\newcommand{\seE}{{\mbox{\scriptsize\boldmath$E$}}}
%\newcommand{\sfF}{{\mbox{\scriptsize\boldmath$F$}}}
\newcommand{\sgG}{{\mbox{\scriptsize\boldmath$G$}}}
\newcommand{\shH}{{\mbox{\scriptsize\boldmath$H$}}}
\newcommand{\siI}{{\mbox{\scriptsize\boldmath$I$}}}
\newcommand{\sjJ}{{\mbox{\scriptsize\boldmath$J$}}}
\newcommand{\smM}{{\mbox{\scriptsize\boldmath$M$}}}
\newcommand{\snN}{{\mbox{\scriptsize\boldmath$N$}}}
\newcommand{\soO}{{\mbox{\scriptsize\boldmath$O$}}}
\newcommand{\spP}{{\mbox{\scriptsize\boldmath$P$}}}
\newcommand{\sqQ}{{\mbox{\scriptsize\boldmath$Q$}}}
\newcommand{\srR}{{\mbox{\scriptsize\boldmath$R$}}}
\newcommand{\ssS}{{\mbox{\scriptsize\boldmath$S$}}}
\newcommand{\stT}{{\mbox{\scriptsize\boldmath$T$}}}
\newcommand{\suU}{{\mbox{\scriptsize\boldmath$U$}}}
\newcommand{\svV}{{\mbox{\scriptsize\boldmath$V$}}}
\newcommand{\swW}{{\mbox{\scriptsize\boldmath$W$}}}
\newcommand{\sxX}{{\mbox{\scriptsize\boldmath$X$}}}
\newcommand{\syY}{{\mbox{\scriptsize\boldmath$Y$}}}
%%
%%
%%
%%
%%                          GRECI
%%
\newcommand{\aalpha}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\bbeta}{{\mbox{\boldmath$\beta$}}}
\newcommand{\ggamma}{{\mbox{\boldmath$\gamma$}}}
\newcommand{\ddelta}{{\mbox{\boldmath$\delta$}}}
\newcommand{\eeta}{{\mbox{\boldmath$\eta$}}}
\newcommand{\llambda}{{\mbox{\boldmath$\lambda$}}}
\newcommand{\mmu}{{\mbox{\boldmath$\mu$}}}
\newcommand{\nnu}{{\mbox{\boldmath$\nu$}}}
\newcommand{\ppi}{{\mbox{\boldmath$\pi$}}}
\newcommand{\rrho}{{\mbox{\boldmath$\rho$}}}
\newcommand{\ssigma}{{\mbox{\boldmath$\sigma$}}}
\newcommand{\ttau}{{\mbox{\boldmath$\tau$}}}
\newcommand{\pphi}{{\mbox{\boldmath$\phi$}}}
\newcommand{\ppsi}{{\mbox{\boldmath$\psi$}}}
\newcommand{\xxi}{{\mbox{\boldmath$ \xi$}}}
\newcommand{\zzeta}{{\mbox{\boldmath$ \zeta$}}}
%%
%%
\newcommand{\saalpha}{{\mbox{\scriptsize\boldmath$\alpha$}}}
\newcommand{\sbbeta}{{\mbox{\scriptsize\boldmath$\beta$}}}
\newcommand{\sggamma}{{\mbox{\scriptsize\boldmath$\gamma$}}}
\newcommand{\sllambda}{{\mbox{\scriptsize\boldmath$\lambda$}}}
\newcommand{\smmu}{{\mbox{\scriptsize\boldmath$\mu$}}}
\newcommand{\snnu}{{\mbox{\scriptsize\boldmath$\nu$}}}
\newcommand{\sttau}{{\mbox{\scriptsize\boldmath$\tau$}}}
\newcommand{\seeta}{{\mbox{\scriptsize\boldmath$\eta$}}}
\newcommand{\sssigma}{{\mbox{\scriptsize\boldmath$\sigma$}}}
\newcommand{\srrho}{{\mbox{\scriptsize\boldmath$\rho$}}}
%%
%%
%%
%%
\newcommand{\ssttau}{{\mbox{\boldmath$\scriptscriptstyle\tau$}}}
\newcommand{\sseeta}{{\mbox{\boldmath$\scriptscriptstyle\eta$}}}
%%
%%
%%
%% SANS SERIF NORMAL
%%
%%
\newcommand{\sfa}{{\sf a}}
\newcommand{\sfb}{{\sf b}}
\newcommand{\sfc}{{\sf c}}
\newcommand{\sfd}{{\sf d}}
\newcommand{\sfe}{{\sf e}}
%\newcommand{\sff}{{\sf f}}
\newcommand{\sfg}{{\sf g}}
\newcommand{\sfh}{{\sf h}}
\newcommand{\sfi}{{\sf i}}
\newcommand{\sfm}{{\sf m}}
\newcommand{\sfn}{{\sf n}}
\newcommand{\sfp}{{\sf p}}
\newcommand{\sfq}{{\sf q}}
\newcommand{\sfr}{{\sf r}}
\newcommand{\sfs}{{\sf s}}
\newcommand{\sft}{{\sf t}}
\newcommand{\sfu}{{\sf u}}
\newcommand{\sfv}{{\sf v}}
\newcommand{\sfx}{{\sf x}}
\newcommand{\sfy}{{\sf y}}
\newcommand{\sfA}{{\sf A}}
\newcommand{\sfB}{{\sf B}}
\newcommand{\sfC}{{\sf C}}
\newcommand{\sfD}{{\sf D}}
\newcommand{\sfE}{{\sf E}}
\newcommand{\sfF}{{\sf F}}
\newcommand{\sfK}{{\sf K}}
\newcommand{\sfP}{{\sf P}}
\newcommand{\sfM}{{\sf M}}
\newcommand{\sfR}{{\sf R}}
\newcommand{\sfS}{{\sf S}}
\newcommand{\sfT}{{\sf T}}
\newcommand{\sfU}{{\sf U}}
\newcommand{\sfV}{{\sf V}}
\newcommand{\sfX}{{\sf X}}
\newcommand{\sfY}{{\sf Y}}
\newcommand{\sfZ}{{\sf Z}}
%%
%%
\newcommand{\fra}{{\frak a}}
\newcommand{\frb}{{\frak b}}
\newcommand{\frc}{{\frak c}}
\newcommand{\frd}{{\frak d}}
\newcommand{\fre}{{\frak e}}
%\newcommand{\frf}{{\frak f}}
\newcommand{\frg}{{\frak g}}
\newcommand{\frh}{{\frak h}}
\newcommand{\frl}{{\frak l}}
\newcommand{\frm}{{\frak m}}
\newcommand{\frv}{{\frak v}}
\newcommand{\frV}{{\frak V}}
\newcommand{\frU}{{\frak U}}
\newcommand{\frx}{{\frak x}}
\newcommand{\fry}{{\frak y}}
\newcommand{\frK}{{\frak K}}
\newcommand{\frC}{{\frak C}}
\newcommand{\frD}{{\frak D}}
\newcommand{\frP}{{\frak P}}
\newcommand{\frM}{{\frak M}}
%%
%%
%%
\newcommand{\rma}{{\mathrm a}}
\newcommand{\rmb}{{\mathrm b}}
\newcommand{\rmc}{{\mathrm c}}
\newcommand{\rmd}{{\mathrm d}}
\newcommand{\rme}{{\mathrm e}}
%\newcommand{\rmf}{{\mathrm f}}
\newcommand{\rmg}{{\mathrm g}}
\newcommand{\rmh}{{\mathrm h}}
\newcommand{\rmi}{{\mathrm i}}
\newcommand{\rmm}{{\mathrm m}}
\newcommand{\rmn}{{\mathrm n}}
\newcommand{\rmp}{{\mathrm p}}
\newcommand{\rmq}{{\mathrm q}}
\newcommand{\rmr}{{\mathrm r}}
\newcommand{\rms}{{\mathrm s}}
\newcommand{\rmt}{{\mathrm t}}
\newcommand{\rmu}{{\mathrm u}}
\newcommand{\rmv}{{\mathrm v}}
\newcommand{\rmx}{{\mathrm x}}
\newcommand{\rmy}{{\mathrm y}}
\newcommand{\rmK}{{\mathrm K}}
\newcommand{\rmC}{{\mathrm C}}
\newcommand{\rmD}{{\mathrm D}}
\newcommand{\rmP}{{\mathrm P}}
\newcommand{\rmM}{{\mathrm M}}
\newcommand{\rmS}{{\mathrm S}}
\newcommand{\rmT}{{\mathrm T}}
\newcommand{\rmU}{{\mathrm U}}
\newcommand{\rmV}{{\mathrm V}}
\newcommand{\rmX}{{\mathrm X}}
\newcommand{\rmY}{{\mathrm Y}}
\newcommand{\rmZ}{{\mathrm Z}}
%%
%%       
%%
%%                                OPERATORI e SIMBOLI PARTICOLARI
%%
%%
%%
\newcommand{\Kliminf}{K\kern-3pt-\kern-2pt\mathop{\rm lim\,inf}\limits}  % Kuratowski liminf di insiemi
\newcommand{\supp}{\mathop{\rm supp}\nolimits}   % supporto 
%\newcommand{\span}{\mathop{\rm span}\nolimits}   % span
\newcommand{\conv}{\mathop{\rm conv}\nolimits}   % involucro convesso
\newcommand{\diam}{\mathop{\rm diam}\nolimits}   % diametro
\newcommand{\argmin}{\mathop{\rm argmin}\limits}   % argmin
\newcommand{\Lip}{\mathop{\rm Lip}\nolimits}          %Lipschitz constant
\newcommand{\interior}{\mathop{\rm int}\nolimits}   % interno relativo
\newcommand{\aff}{\mathop{\rm aff}\nolimits}   % inviluppo affine
%\newcommand{\dim}{\mathop{\rm dim}\nolimits}   % dimensione
\newcommand{\tr}{\mathop{\rm tr}\nolimits}     % traccia
%%
%%       DERIVAZIONE
%%
\renewcommand{\d}{{\mathrm d}}
\newcommand{\dt}{{\d t}}
\newcommand{\ddt}{{\frac \d\dt}}
\newcommand{\dx}{{\d x}}
\newcommand{\pd}[1]{{\partial_{#1}}}
\newcommand{\pdt}{{\pd t}}
\newcommand{\pdx}{{\pd x}}
%%
%%
%%
\newcommand{\restr}[1]{\lower3pt\hbox{$|_{#1}$}}
\newcommand{\topref}[2]{\stackrel{\eqref{#1}}#2}
%%
%%
%%
%%
\newcommand{\Haus}[1]{{\mathscr H}^{#1}}     % Misura di Hausdorff
\newcommand{\Leb}[1]{{\mathscr L}^{#1}}      % Misura di Lebesgue
%%
%%
\newcommand{\la}{{\langle}}                  % brackets
\newcommand{\ra}{{\rangle}}
\newcommand{\down}{\downarrow}              %frecce in su e in giu nei limiti
\newcommand{\up}{\uparrow}
\newcommand{\eps}{\varepsilon}  
\newcommand{\nchi}{{\raise.3ex\hbox{$\chi$}}}
\newcommand{\weakto}{\rightharpoonup}
%%
%%
%%          SPAZI R^n....
%%
%%
\newcommand{\Rd}{{\R^d}}
\newcommand{\Rn}{{\R^n}}
\newcommand{\Rm}{{\R^m}}
\newcommand{\RN}{{\R^N}}
%%
%%
\newcommand{\media}{\mkern12mu\hbox{\vrule height4pt           %
          depth-3.2pt                                 %  da usare
          width5pt}\mkern-16.5mu\int\nolimits}        %  nelle formule
%%
%%
% \newenvironment{Proof}{\removelastskip\par\medskip   % inizio e fine dimostrazione
% \noindent{\em Proof.} \rm}{\penalty-20\null\hfill$\square$\par\medbreak}
% %%
% \newenvironment{Proofx}{\removelastskip\par\medskip  % fine dimostrazione senza quadratino
% \noindent{\em Proof.} \rm}{\par}
%%
\newcommand{\forae}{\text{for a.e.}}
\newcommand{\aein}{\text{a.e.\ in}}
\newcommand{\forevery}{\text{for every }}
%%
%%
%%              COMMENTI ESTERNI AL TESTO
%%
%%
%%                        sul margine:        \comments{....}
%%                        frecca di richiamo: \attention
%%                        frecca di richiamo: \attention
%%                        frecca di richiamo: \attention
%%
  \newcommand{\attention}{{\large%
      \marginpar[\hfill$\Longrightarrow$]{$\Longleftarrow$}}}
\newcommand{\citare}{{\large\marginpar{$\Longleftarrow$
      \small\textit{citare}}}}
%%
\setlength{\marginparwidth}{3cm}
%% 
\newcommand{\comments}[1]{
  \marginpar{\footnotesize\emph{#1}}
  %% \begin{minipage}[t]{2cm}
  %%     \footnotesize\emph{#1}
  %%   \end{minipage}}
}


% \newcommand{\QED}{\rule{2mm}{2mm}}
% %%
% %%                      per concludere un remark
% %% 
% \newcommand{\QEO}{\vbox{\offinterlineskip\hrule
%     \hbox{\vrule\phantom{o}\vrule}\hrule}}
% %%


==> macro_diffusion.tex <==
\newcommand{\MetricSpace}{X}                            %Spazio metrico ambiente
\newcommand{\MS}{\MetricSpace}
\newcommand{\Dist}[2]{\sfd(#1,#2)}                                        %Distanza
\newcommand{\DistSquare}[2]{\sfd^2(#1,#2)}                      %sDistanza al quadrato
\newcommand{\Ball}[2]{B_{#1}(#2)}
\newcommand{\IExp}[2]{\sfE_{#1}(#2)}
%%
%%
\newcommand{\MetricDerivative}[1]{|#1'|}                         %Derivata metrica
\newcommand{\MetricDerivativeSquare}[1]{|#1'|^2}
%%
%%              MACRO PER LA DISCRETIZZAZIONE E LE STIME DELL''ERRORE
%%

%%
\newcommand{\Pc}[2]{\overline{#1}\kern-2pt^{\vphantom 0}_{#2}}
%%
\newcommand{\RelativeEntropy}[2]{\mathrm{Ent}(#1|#2)}
\newcommand{\RE}{\RelativeEntropy}
\newcommand{\RelativeEntropyGamma}[1]{\mathrm{Ent}_\gamma(#1)}
\newcommand{\REG}[1]{\mathrm{Ent}_\gamma(#1)}
\newcommand{\REGname}{\mathrm{Ent}_\gamma}

\newcommand{\RelativeFisher}[1]{\mathrm{I}_\gamma(#1)}
\newcommand{\RF}[1]{\mathrm{I}_\gamma(#1)}
\newcommand{\RFroot}[1]{\mathrm{I}^{1/2}_\gamma(#1)}
\newcommand{\RFname}{\mathrm{I}_\gamma}

\newcommand{\ClosureDomain}{\PP_2(\supp(\gamma))}
\newcommand{\CD}{\ClosureDomain}

\newcommand{\EVI}[4]{\mathrm{EVI}_{#4}(#1,{#2}_W,#3)}


\newcommand{\Identity}{\ii}                             % Identita'
\newcommand{\BorelSets}[1]{\BB(#1)}
\newcommand{\BorelMeasures}[1]{\mathcal M(#1)}
%%
\newcommand{\Probabilities}[1]{\mathscr P(#1)}          % misure di probabilita'
\newcommand{\ProbabilitiesTwo}[1]{\mathscr P_2(#1)}     % misure di probabilita' con momento quadratico finito
%%
\newcommand{\ProbabilitiesReg}[1]{\mathscr P^r(#1)} % misure di probabilita' reg. con momento p finito
%%
\newcommand{\PushForward}[2]{#1_{\#}#2}                 % \PushForward{mappa}{misura} 
%%
%% 
%%   PLAN e PLAN MULTIPLI
%%
\newcommand{\AdmissiblePlanII}[2]{\Gamma(#1,#2)}        %\AdmissiblePlanII{misura1}{misura2}, 
%%                                                       PLAN che hanno misura1 e misura2 come marginali 
%%
\newcommand{\AdmissiblePlanIII}[3]{\Gamma(#1,#2,#3)}    %\AdmissiblePlanIII{misura1}{misura2}{misura3}
%%                                                       PLAN con tre marginali assegnate
%%
\newcommand{\OptimalPlanII}[2]{\Gamma_{o}(#1,#2)}       % \OptimalPlanII{misura1}{misura2}
%%                                                       PLAN ottimali con assegnate marginali
%%
%%
%%
%%    DISTANZA DI WASSERSTEIN
%%
\newcommand{\WassersteinDistance}[2]{\sfd_W(#1,#2)}          %\WassersteinDistance{misura1}{misura2}
%%                                                       Distanza di
%%                                                       Wasserstein
%%                                                       tra le misure
\newcommand{\WD}{\WassersteinDistance}
\newcommand{\WassersteinDistanceSquare}[2]{\sfd_W^2(#1,#2)}  % Distanza
                                % al quadrato
\newcommand{\WDS}{\WassersteinDistanceSquare}
%%
\newcommand{\Cylindrical}[1]{{\rm Cyl}(#1)}                      % Funzioni cilindriche
%%
%%
%%
%%
\newenvironment{comment}
{\begin{quote}
       \rule{.5\textwidth}{.5pt}\ \\
       \footnotesize}
{\\\rule{.5\textwidth}{.5pt}
\end{quote}}

\newcommand{\Dom}[1]{\ensuremath{\mathrm{D}(#1)}}

\newcommand{\MeasTest}[2]{#1(#2)}

\newcommand{\Resolvent}{\sfR}

\newcommand{\LLip}{\mathrm{Lip}_{\rm loc,1}}
